Parallel faceted imaging in radio interferometry via proximal splitting (Faceted HyperSARA): I. Algorithm and simulations

Upcoming radio interferometers are aiming to image the sky at new levels of resolution and sensitivity, with wide-band image cubes reaching close to the Petabyte scale for SKA. Modern proximal optimization algorithms have shown a potential to significantly outperform CLEAN thanks to their ability to inject complex image models to regularize the inverse problem for image formation from visibility data. They were also shown to be parallelizable over large data volumes thanks to a splitting functionality enabling the decomposition of the data into blocks, for parallel processing of block-specific data-fidelity terms involved in the objective function. Focusing on intensity imaging, the splitting functionality is further exploited in this work to decompose the image cube into spatio-spectral facets, and enable parallel processing of facet-specific regularization terms in the objective function, leading to the "Faceted HyperSARA" algorithm. Reliable heuristics enabling an automatic setting of the regularization parameters involved in the objective are also introduced, based on estimates of the noise level, transferred from the visibility domain to the domains where the regularization is applied. Simulation results based on a MATLAB implementation and involving synthetic image cubes and data close to Gigabyte size confirm that faceting can provide a major increase in parallelization capability when compared to the non-faceted approach (HyperSARA).

==> Faceted_HyperSARA_-_I._Algo_and_simulations_arXiv/alg_pdfb.tex <==
\begin{algorithm}[tp]
\small
	\KwData{$(\mathbf{y}_{c,l,b} )_{l,b}$, $l \in \{1, \dotsc, \nband_c \}$, $b \in \{1, \dotsc, \nblock \}$\medskip}
	\KwIn{$\mathbf{X}_c^{(0)}$, $\mathbf{P}_c^{(0)} = \bigl( \mathbf{P}_{c,q}^{(0)} \bigr)_q$, $\mathbf{W}_c^{(0)} = \bigl( \mathbf{W}_{c,q}^{(0)} \bigr)_{q}$, $\mathbf{v}_c^{(0)} = \bigl( \mathbf{v}_{c,l,b}^{(0)} \bigr)_{l,b}$, $\bs{\theta}_c = \big( \bs{\theta}_{c,q} \big)_{1 \le q \le \nfacet}$, $\overline{\bs{\theta}}_c = \big( \overline{\bs{\theta}}_{c,q} \big)_{1 \le q \le \nfacet}$\medskip}
	
	\Parameter{$(\mathbf{D}_{q})_q$, $( \mathbf{U}_{c,l,b})_{l,b}$, $\bs{\varepsilon} = (\varepsilon_{c,l,b})_{l,b}$, $\mu_c$, $(\overline{\mu}_{c, q})_q$, $\tau$, $\zeta$, $(\eta_{c,l})_{1 \leq l \leq \nband}$, $\kappa$, $0 < \npdfbmin < \npdfbmax$, $0 < \relvarpdfb < 1$ \medskip}
	
  	$p \leftarrow 0$; $\xi = +\infty$;
    $\check{\mathbf{X}}_c^{(0)} = \mathbf{X}_c^{(0)}$, $\hat{\mathbf{X}}_c^{(0)} = (\hat{\mathbf{x}}_{c,l}^{(0)})_{1 \le l \le L_c} = \mathbf{FZ}\mathbf{X}_c^{(0)}$\;
    $\mathbf{r}_c^{(0)} = (r_{c,l,b}^{(0)})_{l,b} \in \mathbb{R}^{\nband_c \nblock}$, with $r_{c,l,b}^{(0)} = \norm{\mathbf{y}_{c,l,b} - \bs{\Phi}_{c,l,b} \mathbf{x}_{c,l}^{(0)}}_2$\;
  	
  	\While{$(p < \npdfbmin)$ or $\big[ (p < \npdfbmax)$ and $(\xi > \relvarpdfb $ or $\|\mathbf{r}_c^{(p)}\|_2 > 1.01 \|\bs{\varepsilon}\|_2)\big]$}{

		\tcp{Update low-rankness and sparsity variables}
		
  		split $(\widetilde{\mathbf{X}}_{c,q}^{(p)})_{1 \le q \le \nfacet} = (\widetilde{\mathbf{S}}_q\check{\mathbf{X}}_c^{(p)})_{1 \le q \le \nfacet}$\; \label{alg:eq:broadcast_facet}
		
  		split $(\check{\mathbf{X}}_{c,q}^{(p)})_{1\le q \le \nfacet} = (\mathbf{S}_q \check{\mathbf{X}}_c^{(p)})_{1\le q \le \nfacet}$\;
  		
		\tcp{[Parallel on facet cores]}
		\For{q = 1 \KwTo \nfacet \label{alg:step:start_facet-nuclear}}{
		$\mathbf{P}_{c,q}^{(p+1)} = \bigl( \mathbf{I}_{\widetilde{N}_q \times \widetilde{N}_q} - \prox_{\zeta^{-1} \overline{\mu}_{c, q} \lVert \cdot \rVert_{\ast,\overline{\bs{\theta}}_{c,q} }} \bigr) \bigl( \mathbf{P}_{c,q}^{(p)} + \mathbf{D}_{q} \widetilde{\mathbf{X}}_{c,q}^{(p)} \bigr)$\; \label{alg:step:dual_lr}
		$\widetilde{\mathbf{P}}_{c,q}^{(p+1)} = \mathbf{D}_{q}^\dag \mathbf{P}_c^{(p+1)}$\; \label{alg:step:end_facet-nuclear} 
		
		
		$\mathbf{W}_{c,q}^{(p+1)} = \bigl( \mathbf{I}_{\nwcoefs{}_q \times \nwcoefs{}_q} - \prox_{\kappa^{-1}\mu_c \lVert \cdot \rVert_{2, 1,\bs{\theta}_{c,q}}} \bigr) \bigl( \mathbf{W}_{c,q}^{(p)} + \bs{\Psi}^\dag_q \check{\mathbf{X}}_{c,q}^{(p)} \bigr)$\; \label{alg:step:dual_sparsity}
		$\widetilde{\mathbf{W}}_{c,q}^{(p+1)} = \bs{\Psi}_q \mathbf{W}_{c,q}^{(p+1)}$\; \label{alg:step:end_facet-l21} 
		}	
		
	    \tcp{Update data fidelity variables [data cores]}
  		\For{$l$ = 1 \KwTo $\nband_c$}{
  		    $\hat{\mathbf{x}}^{(p+1)}_{c,l} = \mathbf{FZ} {\mathbf{x}}_{c,l}^{(p)}$\label{alg:eq:fourier}
  		    
  		    split $(\hat{\mathbf{x}}^{(p+1)}_{c,l,b})_{1 \le b \le \nblock} = (\mathbf{M}_{c,l,b} \hat{\mathbf{x}}^{(p+1)}_{c,l})_{1 \le b \le \nblock}$\;
  		    \label{alg:eq:broadcast_fourier}
  	     
  	     
		\For{ $b$ = 1 \KwTo $\nblock$ \label{alg:step:start_data}}{
    		$\mathbf{v}_{c,l,b}^{(p+1)} = \mathbf{U}_{c,l,b} \bigl( \mathbf{I}_{M_{c,l,b}} - \prox^{\mathbf{U}_{c,l,b}}_{\iota_{\mathcal{B}(\mathbf{y}_{c,l,b}, \varepsilon_{c,l,b})}} \bigr) \bigl($\nonl \\  
			%
    		\hfill $ \mathbf{U}_{c,l,b}^{-1}\mathbf{v}_{c,l,b}^{(p)} + \, \mathbf{G}_{c,l,b} (2\hat{\mathbf{x}}_{c,l,b}^{(p+1)}-\hat{\mathbf{x}}_{c,l,b}^{(p)}) \bigr)$\; \label{alg:step:dual_data1}
    		
    		$\widetilde{\mathbf{v}}_{c,l,b}^{(p+1)} = \mathbf{G}_{c,l,b}^\dag \mathbf{v}_{c,l,b}^{(p+1)}$\; \label{alg:step:dual_data2}
            $r_{c,l,b}^{(p+1)} = \norm{\mathbf{y}_{c,l,b} - \mathbf{G}_{c,l,b} \hat{\mathbf{x}}_{c,l,b}^{(p+1)}}_2$\;\label{alg:step:residual}
		}
  		}

		\tcp{Inter node communications}
		\For{l = 1 \KwTo $\nband_c$}{	 
		$\displaystyle \mathbf{a}_{c,l}^{(p)} = \sum_{q=1}^\nfacet \Bigl( \zeta \widetilde{\mathbf{S}}_q^\dag\widetilde{\mathbf{p}}_{c,q,l}^{(p+1)}
			 + \kappa \mathbf{S}_q^\dag \widetilde{\mathbf{w}}_{c,q,l}^{(p+1)} \Bigr) $ \nonl\\
			 $\displaystyle \hfill + \, \eta_{c,l} \mathbf{Z}^\dag \mathbf{F}^\dag \sum_{b} \mathbf{M}_{c,l,b}^\dag \widetilde{\mathbf{v}}_{c,l,b}^{(p+1)} $\; \label{alg:step:aggregate}
	    }
			 
	    \tcp{Update image tiles [on facet cores, in parallel]}
  		$\mathbf{X}_c^{(p+1)} = \prox_{\iota_{\mathbb{R}^{\nbpix \times \nband_c}_+}} \bigl( \mathbf{X}_c^{(p)} - \tau \mathbf{A}_c^{(p)}  \bigr)$\label{alg:step:primal}\tcp*{$\mathbf{A}_c^{(p)} = \big(\mathbf{a}_{c,l}^{(p)} \big)_{1\leq l \leq \nband}$}
  		$\check{\mathbf{X}}_c^{(p+1)} = 2\mathbf{X}_c^{(p+1)} - \mathbf{X}_c^{(p)}$\tcp*{communicate facet borders}

		$\xi = \norm{\mathbf{X}_c^{(p+1)}-\mathbf{X}_c^{(p)}}_\text{F}/\norm{\mathbf{X}_c^{(p)}}_\text{F}$\;
		$p \leftarrow p+1$\;
    }
	\KwResult{
	$\mathbf{X}_c^{(p)}$, $\mathbf{P}_c^{(p)}$, $\mathbf{W}_c^{(p)}$, $\mathbf{v}_c^{(p)}$}
	\caption{
	\label{alg:pdfb}
	Inner convex optimisation algorithm (PDFB) to solve each spectral sub-problem \eqref{eq:problem-split-subcube-approx}.
	}
\end{algorithm}


==> Faceted_HyperSARA_-_I._Algo_and_simulations_arXiv/alg_reweigthing.tex <==
\begin{algorithm}[t]
\small
	\KwData{$(\mathbf{y}_{c,l,b} )_{c,l,b}$, $c \in \{1, \dotsc, C\}$, $l \in \{1, \dotsc, \nband_c \}$, $b \in \{1, \dotsc, \nblock \}$}
	\KwIn{$\mathbf{X}^{(0)} = (\mathbf{X}_c^{(0)})_c$, $\mathbf{P}^{(0)} = (\mathbf{P}_c^{(0)})_c$, $\mathbf{W}^{(0)} = (\mathbf{W}_c^{(0)})_c$, $\mathbf{v}^{(0)} = (\mathbf{v}_c^{(0)})_c$}
	
	\Parameter{$\nreweightmax > 0$, $0 < \relvarrw < 1$}
  	
  	$t \leftarrow 0$, $\xi \leftarrow +\infty$\;
    
    \tcp{Solve spectral sub-problems in parallel}
	\For{$c = 1$ \KwTo $C$ \label{algo:rw:forC}}{
  	\While{$(t < \nreweightmax)$ and $(\xi > \relvarrw)$}{
	
	    \For{$q = 1$ \KwTo $Q$}{
    		\tcp{Update weights (low-rankness prior)}
    		$\overline{\bs{\theta}}_{c,q}^{(t)} =
    		    \overline{\bs{\omega}}_{c,q}(\mathbf{X}_c^{(t)})$; \quad \tcp{using \eqref{eq:facet_hypersara_rank}} \label{alg:step:weights_nuclear}
		    
    		\tcp{Update weights (joint-sparsity prior)}
    		$\bs{\theta}_{c,q}^{(t)} =
    		    \bs{\omega}_{c,q}(\mathbf{X}_c^{(t)})$; \quad \tcp{using \eqref{eq:facet_hypersara_sparsity}}
    		    \label{alg:step:weights_l21}
    	}
  	
  		\tcp{Run PDFB (Algorithm~\ref{alg:pdfb})}
  	    $(\mathbf{X}_c^{(t+1)}, \mathbf{P}_c^{(t+1)}, \mathbf{W}_c^{(t+1)}, \mathbf{v}_c^{(t+1)}) = $\nonl\\
  	    $ \qquad \textbf{Algorithm2}\bigl(\mathbf{X}_c^{(t)}, \mathbf{P}_c^{(t)}, \mathbf{W}_c^{(t)}, \mathbf{v}_c^{(t)}, \bs{\theta}_c^{(t)}, \overline{\bs{\theta}}_c^{(t)}  \bigr) $\; \label{alg:step:pdfb}
    }
    $\xi = \norm{\mathbf{X}_c^{(t+1)}-\mathbf{X}_c^{(t)}}_\text{F}/\norm{\mathbf{X}_c^{(t)}}_\text{F}$\;
	$t \leftarrow t+1$\;
	}	
	\KwResult{$\mathbf{X}^{(t)}$, $\mathbf{P}^{(t)}$, $\mathbf{W}^{(t)}$, $\mathbf{v}^{(t)}$}
	\caption{Outer reweighting algorithm.}
	\label{alg:reweighting}
\end{algorithm}


==> Faceted_HyperSARA_-_I._Algo_and_simulations_arXiv/command_picture.tex <==
% \newcommand{\zoom}[2]{
% \begin{tikzpicture}[
%     node distance = 0cm,
%     inner sep = 0pt,spy using outlines={rectangle, white, magnification=3, every spy on node/.append style={ultra thin},
%     %connect spies,
%     }]
%     \node (n0)  {\includegraphics[keepaspectratio,width=#1]{#2}};
%     \spy [white,size=0.13\textwidth] on (1.1,0.6) in node[above right=of n0.south west, line width=0.1mm];
% \end{tikzpicture}
% }

% \newcommand{\zoom}[2]{
% \begin{tikzpicture}[
%     node distance = 0cm,
%     inner sep = 0pt,spy using outlines={rectangle, white, magnification=3, every spy on node/.append style={ultra thin},
%     %connect spies,
%     }]
%     \node (n0)  {\includegraphics[keepaspectratio,width=#1]{#2}};
%     \spy [white,size=0.13\textwidth] on (1.15,0.35) in node[above right=of n0.south west, line width=0.1mm];
% \end{tikzpicture}
% }

\newcommand{\zoom}[2]{
\begin{tikzpicture}[
    node distance = 0cm,
    inner sep = 0pt,spy using outlines={rectangle, white, magnification=3, every spy on node/.append style={ultra thin},
    %connect spies,
    }]
    \node (n0)  {\includegraphics[keepaspectratio,width=#1]{#2}};
    \spy [white,size=0.08\textwidth] on (0,-0.5) in node[above right=of n0.north west, line width=0.1mm];
\end{tikzpicture}
}

\newcommand{\imdraw}[2]{
\begin{tikzpicture}[
    node distance = 0cm,
    inner sep = 0pt,
    node/.append style={ultra thin},
    ]
    \node[anchor=south west,inner sep=0] at (0,0) (image) {\includegraphics[keepaspectratio,width=#1]{#2}};
    \begin{scope}[x={(image.south east)},y={(image.north west)}]
        \draw[white] (0.48,0.22) rectangle ++(0.12,0.2);
        \draw[white] (0.46,0.75) rectangle ++(0.07,0.25);
        \draw[white] (0.23,0.75) rectangle ++(0.20,0.08);
    \end{scope}
\end{tikzpicture}
}

\newcommand{\zoomgraph}[6]{
\begin{tikzpicture}[
    node distance = 0cm,
    inner sep = 0pt,spy using outlines={rectangle, white, dashed, magnification=3, every spy on node/.append style={ultra thin},connect spies,
    %connect spies,
    }]
    \node (n0)  {\includegraphics[keepaspectratio,width=#1]{#2}};
    \spy [white,width=#3,height=#4] on (#5,#6) in node[above left=of n0.east, line width=0.1mm];
\end{tikzpicture}
}

==> Faceted_HyperSARA_-_I._Algo_and_simulations_arXiv/fig_band_interleaved.tex <==
\begin{figure}
	\centering
	(a) Full image cube \hspace{0.4cm} (b) Spectral sub-cubes \hspace{0.15cm} (c) Facets \& weights\\
	\vspace{0.1cm}
	\includegraphics[keepaspectratio,width=0.45\textwidth]{figs/faceting_illustration.png}
    \caption{Illustration of the proposed faceting scheme, using a 2-fold spectral interleaving process and 9-fold spatial tiling process. The full image cube variable (a) is divided into two spectral sub-cubes (b) with interleaved channels (for a 2-fold interleaving, even and odd channels respectively define a sub-cube). Each sub-cube is spatially faceted. A regular tessellation (dashed red lines) is used to define spatio-spectral tiles. The spatio-spectral facets result from the augmentation of each tile to produce an overlap between facets (solid red lines). Panel (c) shows a single facet (left), as well as the spatial weighting scheme (right) with linearly decreasing weights affecting pixels involved in multiple contiguous facets. Note that, though the same tiling process is underpinning the low-rankness and the average joint sparsity regularization terms, the definition of the appropriate overlap region is specific to each of these terms (\emph{via} the selection operators $\widetilde{\mathbf{S}}_q$ and $\mathbf{S}_q$ in~\eqref{eq:facet_hypersara}).}
    \label{fig:facets}
\end{figure}

==> Faceted_HyperSARA_-_I._Algo_and_simulations_arXiv/fig_blocking.tex <==
\begin{figure}
    \centering
    \hspace{0.3cm} (a) Full data cube \hfill \hspace{0.65cm} (b) Per channel data \hfill (c) Data blocks \hspace{0.2cm} \hfill\\
    \vspace{0.1cm}
    \includegraphics[keepaspectratio,width=0.45\textwidth]{data2.png}
    \caption{Illustration of the data blocking strategy. Starting from the full data cube (a), each of the $\nband$ channels represented in (b) is decomposed into $\nblock$ data blocks (c). The data blocks for each channel are associated with separate data-fidelity terms in the objective function, processed by independent workers.}
    \label{fig:blocking}
\end{figure}


==> Faceted_HyperSARA_-_I._Algo_and_simulations_arXiv/fig_communications.tex <==
\begin{figure}
    \centering
    \begin{subfigure}{0.22\textwidth}
        \centering
        \includegraphics[width=\textwidth,keepaspectratio]{figs/broadcast2.pdf}
        \caption{Broadcast values of the tile before facet update in dual space}
        \label{fig:update_gc}
    \end{subfigure}
    \qquad
    \begin{subfigure}{0.22\textwidth}
        \centering
        \includegraphics[width=\textwidth,keepaspectratio]{figs/aggregate2.pdf}
        \caption{Broadcast and average borders before tile update in primal space
        }
        \label{fig:aggregate_gc}
    \end{subfigure}
    \caption{Illustration of the communication steps involving a facet core (represented by the top-left rectangle in each sub-figure) and a maximum of three of its neighbours. The tile underpinning each facet, located in its bottom-right corner, is delineated in thick black lines. At each iteration, the following two steps are performed sequentially. (a) Facet borders need to be completed before each facet is updated independently in the dual space (Algorithm~\ref{alg:pdfb} lines~\ref{alg:step:start_facet-nuclear}--\ref{alg:step:end_facet-l21}): values of the tile of each facet (top left) are broadcast to cores handling the neighbouring facets in order to update their borders (Algorithm~\ref{alg:pdfb} line~\ref{alg:eq:broadcast_facet}). (b) Parts of the facet tiles overlapping with borders of nearby facets need to be updated before each tile is updated independently in the primal space (Algorithm~\ref{alg:pdfb} line~\ref{alg:step:aggregate}): values of the parts of the borders overlapping with the tile of each facet are broadcast by the cores handling neighbouring facets, and averaged.
    }
    \label{fig:facet_communications}
\end{figure}


==> Faceted_HyperSARA_-_I._Algo_and_simulations_arXiv/fig_overlap.tex <==
\begin{figure*}
    \begin{center}
        \begin{subfigure}{\textwidth}
            \includegraphics[width=0.48\textwidth,keepaspectratio]{figs/synth_spatial/x1}\\
            %
            \includegraphics[width=0.48\textwidth,keepaspectratio]{figs/synth_spatial/x_fhs01}
            \raisebox{-0.45cm}{\includegraphics[width=0.486\textwidth,keepaspectratio]{figs/synth_spatial/res_fhs01}}\\
            %
            \includegraphics[width=0.48\textwidth,keepaspectratio]{figs/synth_spatial/x_fhs1}
            \raisebox{-0.45cm}{\includegraphics[width=0.486\textwidth,keepaspectratio]{figs/synth_spatial/res_fhs1}}\\
            %
            \includegraphics[width=0.48\textwidth,keepaspectratio]{figs/synth_spatial/x_hs1}
            \raisebox{-0.45cm}{\includegraphics[width=0.486\textwidth,keepaspectratio]{figs/synth_spatial/res_hs1}}
        \end{subfigure}
    \end{center}
    
    \vspace*{-0.2cm}
    
    \caption{Spatial faceting experiment: reconstructed images of channel $\nu_{1} = 2.052$ GHz of an image cube with $L=20$ spectral channels, obtained with Faceted HyperSARA (using $(\nfacet,\ncube)=(16,1)$) and HyperSARA (\emph{i.e.} Faceted HyperSARA with $(\nfacet,\ncube)=(1,1)$). Top row: ground truth image (Jy/pixel) displayed in $\log_{10}$ scale. In rows $2-4$ are reported the reconstructed images of Faceted HyperSARA without overlap, Faceted HyperSARA with 10\% overlap and HyperSARA, respectively. From left to right, model image (Jy/pixel) displayed in $\log_{10}$ scale and residual image normalized by $\|\bs{\Phi}_{1}\|_{\text{S}}^2$, displayed in linear scale. Horizontal and vertical marks at the panel edges identify the contour of each tile.}
    \label{fig:images_overlap_1}
\end{figure*}


\begin{figure*}
    \begin{center}
        \begin{subfigure}{\textwidth}
            \imdraw{0.48\textwidth}{figs/synth_spatial/x2}\\
            %
            \imdraw{0.48\textwidth}{figs/synth_spatial/x_fhs02}
            \raisebox{-0.45cm}{\includegraphics[width=0.486\textwidth,keepaspectratio]{figs/synth_spatial/res_fhs02}}\\
            %
            \imdraw{0.48\textwidth}{figs/synth_spatial/x_fhs2}
            \raisebox{-0.45cm}{\includegraphics[width=0.486\textwidth,keepaspectratio]{figs/synth_spatial/res_fhs2}}\\
            %
            \imdraw{0.48\textwidth}{figs/synth_spatial/x_hs2}
            \raisebox{-0.45cm}{\includegraphics[width=0.486\textwidth,keepaspectratio]{figs/synth_spatial/res_hs2}}
        \end{subfigure}
    \end{center}
    
    \vspace*{-0.2cm}
    
    \caption{Spatial faceting experiment: reconstructed images of channel $\nu_{20} = 3.572$ GHz of an image cube with $L=20$ spectral channels, obtained with Faceted HyperSARA ($(\nfacet,\ncube)=(16,1)$) and HyperSARA (\emph{i.e.} Faceted HyperSARA with $(\nfacet,\ncube)=(1,1)$). Top row: ground truth image (Jy/pixel) displayed in $\log_{10}$ scale. In rows $2-4$ are reported the reconstructed images of Faceted HyperSARA without overlap, Faceted HyperSARA with 10\% overlap, and HyperSARA, respectively. From left to right, model image (Jy/pixel) displayed in $\log_{10}$ scale and residual image normalized by $\|\bs{\Phi}_{20}\|_{\text{S}}^2$, displayed in linear scale. Horizontal and vertical marks at the panel edges identify the contour of each tile. In absence of overlap, and in this case only, facet artefacts emerge in the model image obtained with Faceted HyperSARA. Regions where artefacts appear in absence of facet overlap are delineated in white in all the figures to ease the comparison.}
    \label{fig:images_overlap_2}
\end{figure*}


==> Faceted_HyperSARA_-_I._Algo_and_simulations_arXiv/fig_sub.tex <==
\begin{figure*}
    \begin{center}
        \begin{subfigure}{\textwidth}
            \includegraphics[width=0.48\textwidth,keepaspectratio]{figs/synth_spectral/x1}\\
            %
            \includegraphics[width=0.48\textwidth,keepaspectratio]{figs/synth_spectral/x_fhs_Qc11}
            \raisebox{-0.45cm}{\includegraphics[width=0.49\textwidth,keepaspectratio]{figs/synth_spectral/res_fhs_Qc11}}\\
            %
            \includegraphics[width=0.48\textwidth,keepaspectratio]{figs/synth_spectral/x_fhs_Qc101}
            \raisebox{-0.45cm}{\includegraphics[width=0.49\textwidth,keepaspectratio]{figs/synth_spectral/res_fhs_Qc101}}\\
            %
            \includegraphics[width=0.48\textwidth,keepaspectratio]{figs/synth_spectral/x_l11}
            \raisebox{-0.45cm}{\includegraphics[width=0.49\textwidth,keepaspectratio]{figs/synth_spectral/res_l11}}\\
        \end{subfigure}
    \end{center}

    \vspace*{-0.2cm}

    \caption{Spectral faceting experiment: reconstructed images of channel $\nu_{1} = 2.052$ GHz of an image cube with $\nband=100$ spectral channels, obtained with Faceted HyperSARA (using $(\nfacet, \ncube)=(1,10)$), HyperSARA (\emph{i.e.} Faceted HyperSARA with $(\nfacet,\ncube)=(1,1)$) and SARA (\emph{i.e.} Faceted HyperSARA with $(\nfacet, \ncube, (\overline{\mu}_{c, q})_{c,q})=(1, \nband, \mathbf{0}_{\ncube \times \nfacet})$). Top row: ground truth image (Jy/pixel) displayed in $\log_{10}$ scale. In rows $2-4$ are reported the reconstructed images of Faceted HyperSARA, HyperSARA and SARA, respectively. From left to right, model image (Jy/pixel) displayed in $\log_{10}$ scale and residual image normalized by $\|\bs{\Phi}_{1}\|_{\text{S}}^2$, displayed in linear scale.}
    \label{fig:images_sub_1}
\end{figure*}


\begin{figure*}
    \begin{center}
        \begin{subfigure}{\textwidth}
            \includegraphics[width=0.48\textwidth,keepaspectratio]{figs/synth_spectral/x2}\\
            %
            \includegraphics[width=0.48\textwidth,keepaspectratio]{figs/synth_spectral/x_fhs_Qc12}
            \raisebox{-0.45cm}{\includegraphics[width=0.49\textwidth,keepaspectratio]{figs/synth_spectral/res_fhs_Qc12}}\\
            %
            \includegraphics[width=0.48\textwidth,keepaspectratio]{figs/synth_spectral/x_fhs_Qc102}
            \raisebox{-0.45cm}{\includegraphics[width=0.49\textwidth,keepaspectratio]{figs/synth_spectral/res_fhs_Qc102}}\\
            %
            \includegraphics[width=0.48\textwidth,keepaspectratio]{figs/synth_spectral/x_l12}
            \raisebox{-0.45cm}{\includegraphics[width=0.49\textwidth,keepaspectratio]{figs/synth_spectral/res_l12}}
        \end{subfigure}
    \end{center}

    \vspace*{-0.2cm}

    \caption{Spectral faceting experiment: reconstructed images of channel $\nu_{100} = 3.636$ GHz of an image cube with $\nband=100$ spectral channels, obtained with Faceted HyperSARA (using $(\nfacet, \ncube)=(1,10)$), HyperSARA (\emph{i.e.} Faceted HyperSARA with $(\nfacet,\ncube)=(1,1)$) and SARA (\emph{i.e.} Faceted HyperSARA with $(\nfacet, \ncube, (\overline{\mu}_{c, q})_{c,q})=(1, \nband, \mathbf{0}_{\ncube \times \nfacet})$). Top row: ground truth image (Jy/pixel) displayed in $\log_{10}$ scale. In rows $2-4$ are reported the reconstructed images of Faceted HyperSARA, HyperSARA and SARA, respectively. From left to right, model image (Jy/pixel) displayed in $\log_{10}$ scale and residual image normalized by $\|\bs{\Phi}_{100}\|_{\text{S}}^2$, displayed in linear scale.}
    \label{fig:images_sub_2}
\end{figure*}


==> Faceted_HyperSARA_-_I._Algo_and_simulations_arXiv/tab_facets.tex <==
\begin{table*}
    \centering
    \resizebox{0.98\textwidth}{!}{%
    \begin{tabular}{lrrrrrrrr} \toprule
        & $\aSNR$ ($\pm \sSNR$) (dB)  & $\aSNR_{\log}$ ($\pm \sSNR_{\log}$) (dB) & CPU cores & PDFB iterations & $\runp$ (s) & $\run$ (h) & $\cpup$ (s) & $\cpu$ (h) \\ \midrule
        SARA
        & \textbf{35.05 ($\pm 5.90e-01$)} & 13.72 ($\pm 1.59e-01$) & 240 & 3275 & \textbf{3.28 ($\pm 3.79e-01$)} & 3.38 & \textbf{7.13 ($\pm 9.50e-01$)} & 129.77 \\
        HyperSARA
        & \textbf{39.47 ($\pm  2.15e+00$)} & 16.36 ($\pm 1.27e+00$) & 22  & 9236 & \textbf{25.36 ($\pm 8.51e-01$)} & 65.06 & \textbf{84.49 ($\pm 2.79e+00$)} & 216.76 \\
        Faceted HyperSARA ($\nfacet=4$)
        & \textbf{39.79 ($\pm 2.34e+00$)} & 16.47 ($\pm 1.39e+00$) & 24 & 10989  & \textbf{26.50 ($\pm 1.88e+00$)} & 80.90 & \textbf{184.41 ($\pm 9.22e+00$)} & 562.90 \\
        Faceted HyperSARA ($\nfacet=9$)
        & \textbf{40.00 ($\pm 2.40e+00$)} & 16.82 ($\pm 1.42e+00$) & 29 & 11009 & \textbf{15.38 ($\pm 1.38e+00$)} & 47.04 & \textbf{226.52($\pm 1.10e+01$)} & 692.71 \\
        Faceted HyperSARA ($\nfacet=16$)
        & \textbf{ 40.08 ($\pm 2.40e+00$)} & 16.85 ($\pm 1.43e+00$) & 36 & 10945 & \textbf{11.62 ($\pm 4.97e-01$)} & 35.32 & \textbf{286.06 ($\pm 1.08e+01$)} & 869.71  \\
        \bottomrule
    \end{tabular}
    }
    \caption{Spatial faceting experiment: varying number of facets along the spatial dimension $\nfacet$. Reconstruction performance of Faceted HyperSARA ($\ncube=1$, overlap of 10\%), compared to HyperSARA (\emph{i.e.} Faceted HyperSARA with $(\nfacet,\ncube)=(1, 1)$) and SARA (\emph{i.e.} Faceted HyperSARA with $(\nfacet, \ncube, (\overline{\mu}_{c, q})_{c,q})=(1, \nband, \mathbf{0}_{\ncube \times \nfacet})$). The results are reported in terms of
    average $\aSNR$ and $\aSNR_{\log}$ (both in dB, with the associated standard deviation over frequencies $\sSNR$ and $\sSNR_{\log}$), runtime and CPU time per iteration per sub-cube ($\runp$ and $\cpup$ in seconds, with the associated standard deviation over the iterations and the $C$ spectral subcubes). The number of CPU cores, the total number of PDFB iterations until convergence and the total runtime and CPU time to reconstruct the full image cube are also reported. The reconstruction $\SNR$ and the runtime per iteration are highlighted in bold face.} 
    \label{tab:facet_number}
\end{table*}


==> Faceted_HyperSARA_-_I._Algo_and_simulations_arXiv/tab_notations.tex <==
\begin{table}
    \centering
    \caption{Problem dimensions and mathematical notations}
    \label{tab:maths_notations}
    \begin{tabular}{ll} \toprule
        \multicolumn{2}{l}{\emph{Problem dimensions}} \\ \midrule
        $\nbpix$ & image size \\
        $\nfourier$ & size of the 2D oversampled Fourier space \\
        $\nblock$ & number of data blocks per channel \\
        $\nband$ & number of spectral channels \\
        $\ndata$ & number of visibilities \\
        $\ncube$ & number of spectral sub-cubes \\
        $\nfacet$ & number of spatial facets \\ \midrule
        \multicolumn{2}{l}{\emph{Mathematical notations}} \\ \midrule
        $\mathbf{I}_{\ndata \times \ndata}$ & identity matrix, of size $\ndata \times \ndata$ \\
        $\mathbf{0}_{\ndata}$ & vector of size $\ndata$ whose entries are all equal to 0\\
        $\mathbf{0}_{\ncube \times \nfacet}$ & matrix of size $\ncube \times \nfacet$ whose entries are all equal to 0\\
        $[\mathbf{Z}]_i$ & $i$th row of the matrix $\mathbf{Z}$ \\
        $[\mathbf{Z}]_{i,j}$ & element in position $(i,j)$ of the matrix $\mathbf{Z}$ \\
        $\mathbf{Z}^\dagger$ & adjoint (conjugate transpose) of the matrix $\mathbf{Z}$ \\
        $\sgn$ & element-wise sign function \\
        $\iota_C$ & indicator function of the set $C$ \\
        $\vert \cdot \vert$ & element-wise absolute value \\
        $\Vert \cdot \Vert_{\text{S}}$ & spectral norm of a linear operator \\
        $\Vert \cdot \Vert_{*}$ & nuclear norm \\
        $\Vert \cdot \Vert_{2,1}$ & $\ell_{2,1}$ norm \\
        $\Vert \cdot \Vert_{*,\overline{\bs{\omega}}}$ & weighted nuclear norm, with weights $\overline{\bs{\omega}}$ (see~\eqref{eq:weighted_nuclear_norm}) \\
        $\Vert \cdot \Vert_{2,1,\bs{\omega}}$ & weighted $\ell_{2,1}$ norm, with weights $\bs{\omega}$ (see~\eqref{eq:weighted_l21_norm}) \\
        \bottomrule
    \end{tabular}
\end{table}


==> Faceted_HyperSARA_-_I._Algo_and_simulations_arXiv/tab_overlap.tex <==
\begin{table*}
    \centering
    \resizebox{0.98\textwidth}{!}{%
    \begin{tabular}{lrrrrrrrr} \toprule
        & $\aSNR$ ($\pm \sSNR$) (dB)  & $\aSNR_{\log}$ ($\pm \sSNR_{\log}$) (dB) & CPU cores & PDFB iterations & $\runp$ (s) & $\run$ (h) & $\cpup$ (s) & $\cpu$ (h) \\ \midrule
        SARA
        & \textbf{35.05 ($\pm 5.90e-01$)} & 13.72 ($\pm 1.59e-01$) & 240 & 3275 & \textbf{3.28 ($\pm 3.79e-01$)} & 3.38 & \textbf{7.13 ($\pm 9.50e-01$)} & 129.77 \\
        HyperSARA
        & \textbf{39.47 ($\pm  2.15e+00$)} & 16.36 ($\pm 1.27e+00$) & 22  & 9236 & \textbf{25.36 ($\pm 8.51e-01$)} & 65.06 & \textbf{84.49 ($\pm 2.79e+00$)} & 216.76 \\
        Faceted HyperSARA (0\% overlap)
        & \textbf{40.03 ($\pm 2.41e+00$)} & 16.79 ($\pm 1.42e+00$) & 36 & 10961 & \textbf{11.55 ($\pm 7.03e-01$)} & 35.18 & \textbf{284.17 ($\pm 1.34e+01$)} & 865.22 \\
        Faceted HyperSARA (10\% overlap)
        & \textbf{ 40.08 ($\pm 2.40e+00$)} & 16.85 ($\pm 1.43e+00$) & 36 & 10945 & \textbf{11.62 ($\pm 4.97e-01$)} & 35.32 & \textbf{286.06 ($\pm 1.08e+01$)} & 869.71  \\
        Faceted HyperSARA (25\% overlap)
        & \textbf{40.22 ($\pm 2.41e+00$)} & 16.96 ($\pm 1.47e+00$) & 36 & 10918 &  \textbf{11.96 ($\pm 5.34e-01$)} & 36.26 & \textbf{290.71 ($\pm 1.39e+01$)} & 881.66 \\
        Faceted HyperSARA (40\% overlap)
        & \textbf{40.24 ($\pm 2.42e+00$)} & 17.05 ($\pm 1.51e+00$) & 36 & 10934 & \textbf{12.67 ($\pm 5.45e-01$)} & 38.47 & \textbf{298.32 ($\pm 1.43e+01$)} & 906.08 \\ 
        Faceted HyperSARA (50\% overlap)
        & \textbf{40.08 ($\pm 2.53e+00$)} & 16.95 ($\pm 1.52e+00$) & 36 & 10962 & \textbf{13.69 ($\pm 6.48e-01$)} & 41.68 & \textbf{311.14 ($\pm 1.60e+01$)} & 947.41 \\ 
        \bottomrule 
    \end{tabular}
    }
    \caption{Spatial faceting experiment: varying size of the overlap region for the faceted nuclear norm regularization. Reconstruction performance of Faceted HyperSARA with $(\nfacet, \ncube)=(16, 1)$, compared to HyperSARA (\emph{i.e.} Faceted HyperSARA with $(\nfacet, \ncube)=(1,1)$) and SARA (\emph{i.e.} Faceted HyperSARA with $(\nfacet, \ncube, (\overline{\mu}_{c, q})_{c,q})=(1, \nband, \mathbf{0}_{\ncube \times \nfacet})$). The results are reported in terms of
    average $\aSNR$ and $\aSNR_{\log}$ (both in dB with the associated standard deviation $\sSNR$ and $\sSNR_{\log}$), runtime and CPU time per iteration per sub-cube ($\runp$ and $\cpup$ in seconds, with the associated standard deviation over the iterations and the $\ncube$ spectral subcubes). The number of CPU cores, the total number of PDFB iterations until convergence and the total runtime and CPU time to reconstruct the full image cube are also reported. The reconstruction $\SNR$ and the runtime per iteration are highlighted in bold face.}
    \label{tab:facet_overlap}
\end{table*}


==> Faceted_HyperSARA_-_I._Algo_and_simulations_arXiv/tab_prox.tex <==
\begin{table*}
    \centering
    \caption{Proximal operators involved in Algorithm~\ref{alg:pdfb}.}
    \begin{tabular}{@{}ll@{}}\toprule
        \textbf{Proximal operator for} $\alpha>0$ & \textbf{Description} \\ \midrule
        $\prox_{\alpha \norm{\cdot}_1} (\mathbf{z}) = \sgn(\mathbf{z}) \max \bigl\{\lvert \mathbf{z} \rvert - \alpha, \mathbf{0} \bigr\}$ & $\mathbf{z} \in \mathbb{R}^\nbpix$, soft-thresholding operator \\
        $\prox_{\alpha \norm{\cdot}_{*}} (\mathbf{Z}) = \mathbf{U} \Diag \bigr(\prox_{\alpha \norm{\cdot}_1} (\bs{\sigma}) \bigl) \mathbf{V}^\dag$ & $\mathbf{Z} = \mathbf{U}\bs{\Sigma}\mathbf{V}^\dag \in \mathbb{R}^{\nbpix \times \nband}$, $\bs{\Sigma} = \Diag(\bs{\sigma})$\\
        & singular value decomposition of $\mathbf{Z}$\\
        %
        $\prox_{\alpha \norm{\cdot}_{2, 1}} (\mathbf{Z}) = \Bigl( \max \bigl\{ \norm{\mathbf{z}_n^\dagger}_2 - \alpha, 0 \bigr\} \frac{\mathbf{z}_n^\dagger}{\norm{\mathbf{z}_n^\dagger}_2} \Bigr)_{1 \leq n \leq \nbpix}$ & $\mathbf{Z} = [\mathbf{z}_1, \dotsc, \mathbf{z}_\nbpix]^\dag \in \mathbb{R}^{\nbpix \times \nband}$\\[0.25cm]
        %
        $\prox_{\iota_{\mathcal{B}(\mathbf{y}_{c,l,b}, \varepsilon_{c,l,b})}} (\mathbf{z}) 
        = \dfrac{\mathbf{z} - \mathbf{y}_{c,l,b}}{\max \big\{ \| \mathbf{z} - \mathbf{y}_{c,l,b} \|_2/\varepsilon_{c,l,b}, 1 \big\} } + \mathbf{y}_{c,l,b}$
        & $\mathbf{z} \in \mathbb{C}^{M_{c,l,b}}$\\[0.25cm]
        $\prox_{\iota_{\mathbb{R}^{\nbpix \times \nband}_+}} (\mathbf{Z}) = \max \bigl\{\mathbf{0}, \Re(\mathbf{Z}) \big\}$ & $\mathbf{Z} \in \mathbb{C}^{\nbpix \times \nband}$, $\Re(\mathbf{Z})$ denotes the real part of $\mathbf{Z}$\\ \bottomrule
    \end{tabular}
    \label{tab:proximity}
\end{table*}


==> Faceted_HyperSARA_-_I._Algo_and_simulations_arXiv/tab_spectral.tex <==
\begin{table*}
    \centering
    \resizebox{0.98\textwidth}{!}{%
        \begin{tabular}{lrrrrrrrr} \toprule
            & $\aSNR$ ($\pm \sSNR$) (dB)  & $\aSNR_{\log}$ ($\pm \sSNR_{\log}$) (dB) & CPU cores & PDFB iterations & $\runp$ (s) & $\run$ (h) & $\cpup$ (s) & $\cpu$ (h) \\ \midrule
            SARA
            & \textbf{19.76 ($\pm 3.19e+00$)} & $19.85 (\pm 1.80e+00$) & 1200 & 2205 & \textbf{0.55 ($\pm 4.59e-02$)} & 0.41 & \textbf{0.87 ($\pm 5.56e-02$)}  & 53.01 \\
            HyperSARA
            & \textbf{22.27 ($\pm 2.56e+00$)} & 23.57 ($\pm 1.29e-01$) & 16 & 3800 & \textbf{11.30 ($\pm 1.01e+00$)} & 12.01 & \textbf{64.71 ($\pm 2.42e+00$)} & 68.75 \\
            Faceted HyperSARA ($\ncube = 2$)
            & \textbf{21.77 ($\pm 2.51e+00$)} & 23.37 ($\pm 1.19e-00$) & 32 & 2400 & \textbf{5.68 ($\pm 4.49e-01$)} & 3.80 & \textbf{32.25 ($\pm 1.72e+00$)} & 43.18 \\
            Faceted HyperSARA ($\ncube = 5$)
            & \textbf{21.85 ($\pm 2.72e+00 $)} & 24.73 ($\pm 6.12e-01$) & 80 & 2380 & \textbf{2.67 ($\pm 4.35e-01$)} & 2.01 & \textbf{13.78 ($\pm 1.17e+00$)} & 45.74 \\
            Faceted HyperSARA ($\ncube = 10$)
            & \textbf{22.04 ($\pm 2.85e+00 $)} & 25.03 ($\pm 3.97e-01$) & 160 & 2540 & \textbf{1.53 ($\pm 2.90e-01$)} & 1.36 & \textbf{7.04 ($\pm 9.10e-01$)} & 49.58 \\
            \bottomrule
        \end{tabular}
    }
    \caption{Spectral faceting experiment: reconstruction performance of Faceted HyperSARA with a varying number of spectral sub-problems $\ncube$ and $\nfacet=1$, compared to HyperSARA (\emph{i.e.} Faceted HyperSARA with $(\nfacet,\ncube)=(1,1)$) and SARA (\emph{i.e.} Faceted HyperSARA with $(\nfacet, \ncube, (\overline{\mu}_{c, q})_{c,q})=(1, \nband, \mathbf{0}_{\ncube \times \nfacet})$). The results are reported in terms of
    average $\aSNR$ and $\aSNR_{\log}$ (both in dB with the associated standard deviation $\sSNR$ and $\sSNR_{\log}$), runtime and CPU time per iteration per sub-cube ($\runp$ and $\cpup$ in seconds, with the associated standard deviation over the iterations and the $C$ spectral subcubes). The number of CPU cores, the average number of PDFB iterations across all sub-problems until convergence and the total runtime and CPU time to reconstruct the full image cube are also reported. Note that the runtime and CPU time per iteration are reported as an average over all the sub-problems (since the solvers can be applied independently to distinct sub-problems). The total runtime is defined as the total amount of time needed to reconstruct the full image cube (\emph{i.e.}, the largest runtime taken by the compared methods over all the reconstructed sub-cubes). The reconstruction $\SNR$ and the runtime per iteration are highlighted in bold face.}
    \label{tab:spectral_faceting}
\end{table*}

